Scaling Autonomous Agents via Automatic Reward Modeling And Planning

Large language models (LLMs) have demonstrated remarkable capabilities across a range of text-generation tasks. However, LLMs still struggle with problems requiring multi-step decision-making and environmental feedback, such as online shopping, scientific reasoning, and mathematical problem-solving. Unlike pure text data, collecting large-scale decision-making data is challenging. Moreover, many powerful LLMs are only accessible through APIs, which hinders their fine-tuning for agent tasks due to cost and complexity. To address LLM agents' limitations, we propose a framework that can automatically learn a reward model from the environment without human annotations. This model can be used to evaluate the action trajectories of LLM agents and provide heuristics for task planning. Specifically, our approach involves employing one LLM-based agent to navigate an environment randomly, generating diverse action trajectories. Subsequently, a separate LLM is leveraged to assign a task intent and synthesize a negative response alongside the correct response for each trajectory. These triplets (task intent, positive response, and negative response) are then utilized as training data to optimize a reward model capable of scoring action trajectories. The effectiveness and generalizability of our framework are demonstrated through evaluations conducted on different agent benchmarks. In conclusion, our proposed framework represents a significant advancement in enhancing LLM agents' decision-making capabilities. By automating the learning of reward models, we overcome the challenges of data scarcity and API limitations, potentially revolutionizing the application of LLMs in complex and interactive environments. This research paves the way for more sophisticated AI agents capable of tackling a wide range of real-world problems requiring multi-step decision-making.

==> ICLR_2025_Template/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}
\newcommand{\rebuttal}[1]{\textcolor{blue}{#1}}

% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> ICLR_2025_Template/sections/1_intro.tex <==
\section{Introduction}

Developing AI agents capable of perceiving environments, understanding instructions, and acting to accomplish a wide range of tasks in interactive settings~\citep{1087032} have many real-world applications, including virtual human assistants~\citep{reed2022generalistagent,casheekar2024contemporary}, business process management~\citep{kirchdorfer2024agentsimulator}, and robotic process automation~\citep{rana2023sayplan,saycan2022arxiv,dipalo2023unifiedagentfoundationmodels}.

The recent advent of large generative models has revolutionized numerous applications, such as question answering~\citep{rajpurkar2016squad100000questionsmachine}, text summarization~\citep{NIPS2015_afdec700}, and multi-modal understanding~\citep{chen2015microsoftcococaptionsdata,balanced_vqa_v2,yu2016modelingcontextreferringexpressions}. However, while these models excel in text comprehension and generation tasks, their performance in decision-making scenarios—such as online shopping and scientific reasoning falls relative short of human capabilities.
This disparity likely stems from the nature of the training data. Large generative models are typically pre-trained on readily available image and text corpora from the internet. In contrast, trajectory data for agent tasks, which require multi-step interaction with the environment, is more challenging to collect and does not naturally occur on the internet.
Furthermore, current state-of-the-art commercial Language Learning Models (LLMs), such as GPT-4V~\citep{openai2024gpt4technicalreport} and Gemini~\citep{reid2024gemini}, often provide only limited APIs for general users. This restriction renders it either infeasible or cost-prohibitive to fine-tune these models for specific agent tasks, further impeding progress in this field.

\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth]{figures/teaser.pdf}
   \caption{
   In Fig.~\ref{fig:teaser}~(a), we show that it is difficult for LLM agents to generate multi-step plans in an interactive environment to achieve the instruction goal. However, it is relatively easy for an LLM to learn a reward model that can evaluate whether the trajectories meet the task instructions, as shown in Fig.~\ref{fig:teaser}~(b). In Fig.~\ref{fig:teaser}~(c), we show that a learned reward model can be used to guide the default policy models to improve action planning.}
   \label{fig:teaser}
\end{figure*}


Previous studies have explored the development of autonomous agents for decision-making tasks using large language models (LLMs). Early research~\citep{yao2023webshopscalablerealworldweb,zheng2024seeact,deng2024mind2web} utilized instruction prompts with few-shot examples to direct LLMs in handling various agent tasks. These methods do not require task-specific fine-tuning but have shown limited performance on benchmarks requiring interaction with environments and precise action prediction. A different research direction involves collecting human preference data~\citep{hong2023cogagent} or distilling trajectory data from advanced commercial LLM APIs~\citep{zeng2023agenttuning,deng2024mind2web} and fine-tuning smaller open-source LLMs to create new policy models for agent tasks. However, this distillation process relies on advanced pre-trained agent models for trajectory data extraction, which are often unavailable, expensive, or subject to commercial restrictions. For instance, data from models such as GPT-4 or Gemini cannot be used for commercial purposes.

A fundamental premise of our approach is that, in most agent applications, evaluation is easier than generation~\citep{karp1975computational,naor1996evaluation}. As illustrated in Fig.~\ref{fig:teaser}~(a), \textit{\textbf{generating}} a correct multi-step solution to navigate to the target page is challenging since it needs to predict multiple actions and interact with the environment. However, it is relatively simple to \textit{\textbf{evaluate}} whether the output action trajectories and environment states meet the provided intent to find a \textit{"vans sport canvas fashion sneaker"}. Building on this premise, we suggest that developing a reward model is more feasible than creating a policy model for agent tasks. With an effective reward model, it becomes possible to guide LLMs in planning tasks both effectively and efficiently. For instance, as depicted in Fig.~\ref{fig:teaser}~(c), by integrating the reward model with an LLM-based agent and the Monte Carlo Tree Search (MCTS) algorithm~\citep{silver2017mastering,coulom2006efficient}, we can simulate and evaluate the future states of agent tasks, thereby making better decisions for subsequent actions. This approach is analogous to mental simulation~\citep{hegarty2004mechanical,lake2017building} in cognitive science, where humans envision the outcomes of potential actions to make better decisions in problem-solving.%~\zf{need update fig description.}

While reward models can assist LLM agents in planning, developing these reward models presents significant challenges. Some prior studies have utilized powerful commercial LLM APIs as evaluators for tasks~\citep{kwon2023rewarddesignlanguagemodels}. Although these approaches have demonstrated effectiveness in certain applications, they rely on state-of-the-art LLM models for evaluation, which are often expensive and difficult to scale. In this paper, we introduce an automated method to learn multi-modal reward models without relying on state-of-the-art LLMs for guidance. Furthermore, previous work has not considered integrating the learned reward models with various planning algorithms for problem-solving.

The process of learning the reward model involves three steps. Initially, we utilize an LLM-based agent (e.g.,~\cite{dubey2024llama3herdmodels}) to navigate in the environments, aiming to achieve a randomly proposed intent while collecting extensive action trajectory demonstrations. Subsequently, the LLM model examines the collected trajectories and proposes a refined intent that the sampled trajectories actually accomplish. Additionally, we prompt the LLM to generate negative trajectories that fail to achieve the intended task. Finally, based on the synthetic data (intents, positive trajectories, and negative trajectories) collected, we train a customized reward model using widely adopted vision-language models such as VILA~\citep{lin2023vila} to evaluate whether the user's intent has been fulfilled by the action trajectories. With this automatic reward model, we enhance the performance of LLM-based agents in conjunction with various planning algorithms such as best of n, reflexion, and MCTS.

In summary, we introduce a novel framework \Model (autonomous Agents from automatic Reward Modeling And Planning) for LLM-based agents incorporating an automatic reward model that evaluates task completion, analogous to mental simulation in human cognition. This framework offers several advantages: (1) Effectiveness: It enhances the performance of various LLM agents across different tasks. (2) Flexibility: It eliminates the need for fine-tuning the LLMs themselves and allows for optimization of custom reward targets during inference, enabling more controllable generation.
(3) Practicality: The training of the automatic reward model does not rely on labor-intensive labeling or state-of-the-art commercial LLMs, making it more feasible and widely applicable.

==> ICLR_2025_Template/sections/2_related.tex <==
\section{Related Work}

\paragraph{LLMs for Agent tasks.}

Our research is related to deploying large language models (LLMs) as agents for decision-making tasks in interactive environments~\citep{liu2023agentbench,zhou2023webarena,shridhar2020alfred,toyama2021androidenv}. Earlier works, such as~\citep{yao2023webshopscalablerealworldweb}, fine-tuned models like BERT~\citep{devlin2019bertpretrainingdeepbidirectional} for decision-making in simplified environments, such as online shopping or mobile phone manipulation. With the advent of large language models~\citep{brown2020languagemodelsfewshotlearners,openai2024gpt4technicalreport}, it became feasible to perform decision-making tasks through zero-shot or few-shot in-context learning. To better assess the capabilities of LLMs as agents, several models have been developed~\citep{deng2024mind2web,xiong2024watch,hong2023cogagent,yan2023gpt}. Most approaches~\citep{zheng2024seeact,deng2024mind2web} provide the agent with observation and action history, and the language model predicts the next action via in-context learning. Additionally, some methods~\citep{zhang2023building,li2023camel,song2024trial} attempt to distill trajectories from state-of-the-art language models to train more effective policy models. In contrast, our paper introduces a novel framework that automatically learns a reward model from LLM agent navigation, using it to guide the agents in making more effective plans.

\textbf{LLM Planning.} Our paper is also related to planning with large language models. Early researchers~\citep{brown2020languagemodelsfewshotlearners} often prompted large language models to directly perform agent tasks. Later, \citet{yao2022react} proposed ReAct, which combined LLMs for action prediction with chain-of-thought prompting~\citep{wei2022chain}. Several other works~\citep{yao2023treethoughtsdeliberateproblem,hao2023reasoning,zhao2023large,qiao2024agentplanningworldknowledge} have focused on enhancing multi-step reasoning capabilities by integrating LLMs with tree search methods. Our model differs from these previous studies in several significant ways. First, rather than solely focusing on text generation tasks, our pipeline addresses multi-step action planning tasks in interactive environments, where we must consider not only historical input but also multimodal feedback from the environment. Additionally, our pipeline involves automatic learning of the reward model from the environment without relying on human-annotated data, whereas previous works rely on prompting-based frameworks that require large commercial LLMs like GPT-4~\citep{openai2024gpt4technicalreport} to learn action prediction. Furthermore, \Model supports a variety of planning algorithms beyond tree search.

\textbf{Learning from AI Feedback.} In contrast to prior work on LLM planning, our approach also draws on recent advances in learning from AI feedback~\citep{bai2022constitutional,lee2023rlaif,yuan2024self,sharma2024critical,pan2024autonomous,koh2024tree}. These studies initially prompt state-of-the-art large language models to generate text responses that adhere to predefined principles and then potentially fine-tune the LLMs with reinforcement learning. Like previous studies, we also prompt large language models to generate synthetic data. However, unlike them, we focus not on fine-tuning a better generative model but on developing a classification model that evaluates how well action trajectories fulfill the intended instructions. This approach is simpler, requires no reliance on state-of-the-art LLMs, and is more efficient. We also demonstrate that our learned reward model can integrate with various LLMs and planning algorithms, consistently improving their performance.

\textbf{Inference-Time Scaling.} ~\citet{snell2024scaling} validates the efficacy of inference-time scaling for language models. Based on inference-time scaling, various methods have been proposed, such as random sampling~\citep{wang2022self} and tree-search methods~\citep{hao2023reasoning, zhang2024accessing, guan2025rstar}. Concurrently, several works have also leveraged inference-time scaling to improve the performance of agentic tasks. ~\citet{koh2024tree} adopts a training-free approach, employing MCTS to enhance policy model performance during inference and prompting the LLM to return the reward. ~\citet{gu2024your} introduces a novel speculative reasoning approach to bypass irreversible actions by leveraging LLMs or VLMs. It also employs tree search to improve performance and prompts an LLM to output rewards. ~\citet{yu2024exact} proposes Reflective-MCTS to perform tree search and fine-tune the GPT model, leading to improvements in ~\citet{koh2024visualwebarena}. ~\citet{putta2024agent} also utilizes MCTS to enhance performance on web-based tasks such as ~\citet{yao2023webshopscalablerealworldweb} and real-world booking environments. ~\cite{lin2025qlass} utilizes the stepwise reward to give effective intermediate guidance across different agentic tasks. Our work differs from previous efforts in two key aspects: (1) Broader Application Domain. Unlike prior studies that primarily focus on tasks from a single domain, our method demonstrates strong generalizability across web agents, mathematical reasoning, and scientific discovery domains, further proving its effectiveness. (2) Flexible and Effective Reward Modeling. Instead of simply prompting an LLM as a reward model, we finetune a small scale VLM~\citep{lin2023vila} to evaluate input trajectories. %Our reward scores range continuously between 0 and 1, in contrast to existing methods that rely on discrete scoring (e.g., 0 and 1, or 0, 0.5, and 1) through direct LLM prompting.

% Concurrently, several works have also leveraged inference-time scaling to improve the performance of agentic tasks. ~\citet{pan2024autonomous} demonstrates that LLMs and VLMs, such as the GPT series, can function as evaluators or reward models to provide guidance for fine-tuning or reflection, thereby enhancing digital agents. This lays the groundwork for subsequent studies that directly prompt LLMs as reward models. ~\citet{koh2024tree} adopts a training-free approach, employing MCTS to enhance policy model performance during inference. However, it is limited to web environments~\citep{koh2024visualwebarena}. Moreover, its value function relies on prompting an LLM, which is less effective than our proposed method. We validate our approach through ablation studies, demonstrating that our fine-tuned reward model is more effective. ~\citet{gu2024your} introduces a novel speculative reasoning approach to bypass irreversible actions, such as purchasing a product, by leveraging LLMs or VLMs. It also employs tree search to improve performance, but it remains restricted to the web domain~\citep{koh2024visualwebarena, deng2024mind2web}. Additionally, it lacks reward modeling and instead prompts an LLM to output rewards. ~\citet{yu2024exact} proposes Reflective-MCTS to perform tree search and fine-tune the GPT model, leading to improvements in ~\citep{koh2024visualwebarena}. However, this work focuses solely on a single web agent task, and its reward modeling is derived from multi-agent debate, differing from our more effective and efficient reward modeling approach. ~\citet{putta2024agent} also utilizes MCTS to enhance performance, but it is limited to web-based tasks such as ~\citep{yao2023webshopscalablerealworldweb} and real-world booking environments.

==> ICLR_2025_Template/sections/3_model.tex <==
\section{Model}
\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth]{figures/framework_fig2.pdf}
   \caption{
   The pipeline of our \Model framework. We first generate an initial task instruction using LLMs with in-context learning and sample trajectories aligned with the initial language instructions in the environment. Next, we use the LLM to summarize the sampled trajectories and generate refined task instructions that better match these trajectories. We then modify specific actions within the trajectories to perform new actions in the environment, collecting negative trajectories in the process. Using the refined task instructions, along with both positive and negative trajectories, we train a lightweight reward model to distinguish between matching and non-matching trajectories. The learned reward model can then collaborate with various LLM agents to improve task planning.
   }
   \label{fig:pipeline}
\end{figure*}

In this section, we provide a detailed introduction to our framework, autonomous Agents from automatic Reward Modeling And Planning (\Model). The framework includes automated reward data generation in section~\ref{sec:data}, reward model design in section~\ref{sec:model}, and planning algorithms in section~\ref{sec:plan}.

\subsection{Background}
The planning tasks for LLM agents can be typically formulated as a Partially Observable Markov Decision Process (POMDP): $(\mathcal{X}, \mathcal{S}, \mathcal{A}, \mathcal{O}, \mathcal{T})$, where:
\begin{itemize}
    \item $\mathcal{X}$ is the set of text instructions;
    \item $\mathcal{S}$ is the set of environment states;
    \item $\mathcal{A}$ is the set of available actions at each state;
    \item $\mathcal{O}$ represents the observations available to the agents, including text descriptions and visual information about the environment in our setting;
    \item $\mathcal{T}: \mathcal{S} \times \mathcal{A} \rightarrow \mathcal{S}$ is the transition function of states after taking actions, which is given by the environment in our settings. 
\end{itemize}

Given a task instruction $\mathit{x} \in \mathcal{X}$ and the initial environment state $\mathit{s_0} \in \mathcal{S}$, planning tasks require the LLM agents to propose a sequence of actions ${\{a_n\}_{n=1}^{N}}$ that aim to complete the given task, where $a_n \in \mathcal{A}$ represents the action taken at time step $n$, and $N$ is the total number of actions executed in a trajectory.
Following the $n$-th action, the environment transitions to state $\mathit{s_{n}}$, and the agent receives a new observation $\mathit{o_{n}}$. Based on the accumulated state and action histories, the task evaluator determines whether the task is completed.

An important component of our framework is the learned reward model $\mathcal{R}$, which estimates whether a trajectory $h$ has successfully addressed the task:
\begin{equation}
    r = \mathcal{R}(\mathit{x}, h),
\end{equation}
where $h = \{\{a_n\}_{n=1}^N, \{o_n\}_{n=0}^{N}\}$, $\{a_n\}_{n=1}^N$ are the actions taken in the trajectory, $\{o_n\}_{n=0}^{N}$ are the corresponding environment observations, and $r$ is the predicted reward from the reward model.
By integrating this reward model with LLM agents, we can enhance their performance across various environments using different planning algorithms.

\subsection{ Automatic Reward Data Generation.}
\label{sec:data}
To train a reward model capable of estimating the reward value of history trajectories, we first need to collect a set of training language instructions $\{x_m\}_{m=1}^M$, where $M$ represents the number of instruction goals. Each instruction corresponds to a set of positive trajectories $\{h_m^+\}_{m=1}^M$ that match the instruction goals and a set of negative trajectories $\{h_m^-\}_{m=1}^M$ that fail to meet the task requirements. This process typically involves human annotators and is time-consuming and labor-intensive~\citep{christiano2017deep,rafailov2024direct}. As shown in Fig.~\ref{fig:instruction_generation_sciworld} of the Appendix. we automate data collection by using Large Language Model (LLM) agents to navigate environments and summarize the navigation goals without human labels.

\noindent\textbf{Instruction Synthesis.} The first step in data generation is to propose a task instruction for a given observation. We achieve this using the in-context learning capabilities of LLMs. The prompt for instruction generation is shown in Fig.~\ref{fig:instruction_refinement_sciworld} of the Appendix. Specifically, we provide some few-shot examples in context along with the observation of an environment state to an LLM, asking it to summarize the observation and propose instruction goals. In this way, we collect a set of synthesized language instructions $\{x_m^{raw}\}_{m=1}^M$, where $M$ represents the total number of synthesized instructions.

\noindent\textbf{Trajectory Collection.} Given the synthesized instructions $x_m^{raw}$ and the environment, an LLM-based agent is instructed to take actions and navigate the environment to generate diverse trajectories $\{x_m^{raw}, h_m\}_{m=0}^M$ aimed at accomplishing the task instructions. Here, $h_m$ represents the $m$-th history trajectory, which consists of $N$ actions $\{a_n\}_{n=1}^N$ and $N+1$ environment observations $\{o_n\}_{n=0}^N$.
Due to the limited capabilities of current LLMs, the generated trajectories $h_m$ may not always align well with the synthesized task instructions $x_m$. To address this, we ask the LLM to summarize the completed trajectory $h_m$ and propose a refined goal $x_m^r$. This process results in a set of synthesized demonstrations $\{x_m^r, h_m\}_{m=0}^{M_r}$, where $M_r$ is the number of refined task instructions.

\noindent\textbf{Pairwise Data Construction.} 
To train a reward model capable of distinguishing between good and poor trajectories, we also need trajectories that do not satisfy the task instructions. To create these, we sample additional trajectories that differ from $\{x_m^r, h_m\}$ and do not meet the task requirements by modifying actions in $h_m$ and generating corresponding negative trajectories $\{h_m^-\}$. For clarity, we refer to the refined successful trajectories as $\{x_m, h_m^+\}$ and the unsuccessful ones as $\{x_m, h_m^-\}$. These paired data will be used to train the reward model described in Section~\ref{sec:model}, allowing it to estimate the reward value of any given trajectory in the environment.

\subsection{ Reward Model Design.} 
\label{sec:model}
\noindent\textbf{Reward Model Architectures.}
Theoretically, we can adopt any vision-language model that can take a sequence of visual and text inputs as the backbone for the proposed reward model. In our implementation, we use the recent VILA model~\citep{lin2023vila} as the backbone for reward modeling since it has carefully maintained open-source code, shows strong performance on standard vision-language benchmarks like~\citep{fu2023mme,balanced_vqa_v2,hudson2018gqa}, and support multiple image input. 

The goal of the reward model is to predict a reward score to estimate whether the given trajectory $(x_m, h_m)$  has satisfied the task instruction or not, which is different from the original goal of VILA models that generate a series of text tokens to respond to the task query. To handle this problem, we additionally add a fully-connected layer for the model, which linearly maps the hidden state of the last layer into a scalar value. 

\noindent\textbf{Optimazation Target.}
Given the pairwise data that is automatically synthesized from the environments in Section~\ref{sec:data}, we optimize the reward model by distinguishing the good trajectories $(x_m, h^+_m)$ from bad ones $(x_m, h^-_m)$. Following standard works of reinforcement learning from human feedback~\citep{bradley1952rank,sun2023salmon,sun2023aligning}, we treat the optimization problem of the reward model as a binary classification problem and adopt a cross-entropy loss. Formally, we have 
\begin{equation}
    \mathcal{L(\theta)} = -\mathbf{E}_{(x_m,h_m^+,h_m^-)}[\log\sigma(\mathcal{R}_\theta(x_m, h_m^+)-\mathcal{R}_\theta(x_m, h_m^-))],
\end{equation}
where $\sigma$ is the sigmoid function and $\theta$ are the learnable parameters in the reward model $\mathcal{R}$.
By optimizing this target, the reward model is trained to give higher value scores to the trajectories that are closer to the goal described in the task instruction. 

\subsection{ Planning with Large Vision-Langauge Reward Model.}
After getting the reward model to estimate how well a sampled trajectory match the given task instruction, we are able to combine it with different planning algorithms to improve LLM agents' performance. Here, we summarize the typical algorithms we can adopt in this paper.

\noindent\textbf{Best of N.} This is a simple algorithm that we can adopt the learned reward model to improve the LLM agents' performances. We first prompt the LLM agent to generate $n$ different trajectories independently and choose the one with the highest predicted reward score as the prediction for evaluation. Note that this simple method is previously used in natural language generation~\citep{zhang2024improving} and we adopt it in the context of agent tasks to study the effectiveness of the reward model for agent tasks.

\noindent\textbf{Reflexion.} Reflexion~\citep{shinn2024reflexion} is a planning framework that enables large language models (LLMs) to learn from trial-and-error without additional fine-tuning. Instead of updating model weights, Reflexion agents use verbal feedback derived from task outcomes. This feedback is converted into reflective summaries and stored in an episodic memory buffer, which informs future decisions. Reflexion supports various feedback types and improves performance across decision-making, coding, and reasoning tasks by providing linguistic reinforcement that mimics human self-reflection and learning. %This approach yields significant gains over baseline methods in several benchmarks.

\noindent\textbf{MCTS.} 
We also consider tree search-based planning algorithms like Monte Carlo Tree Search (MCTS)~\citep{coulom2006efficient,silver2017mastering} to find the optimal policy. 
There is a tree structure constructed by the algorithm, where each node represents a state and each edge signifies an action.
Beginning at the initial state of the root node, the algorithm navigates the state space to identify action and state trajectories with high rewards, as predicted by our learned reward model. 

The algorithm tracks 1) the frequency of visits to each node and 2) a value function that records the maximum predicted reward obtained from taking action ${a}$ in state ${s}$.
MCTS would visit and expand nodes with either higher values (as they lead to high predicted reward trajectory) or with smaller visit numbers (as they are under-explored).
We provide more details in the implementation details and the appendix section.


\label{sec:plan}

==> ICLR_2025_Template/sections/4_exp.tex <==
\section{Experiments}
In this section, we conduct a series of experiments to demonstrate the effectiveness of the proposed framework for agent tasks. First, we evaluate the framework's performance on standard agent benchmarks~\citep{yao2023webshopscalablerealworldweb,scienceworld2022,yao2023treethoughtsdeliberateproblem}, detailed in Section~\ref{exp:effect}. Next, we show how customizing the reward target during inference allows us to generate more tailored action plans, as described in Section~\ref{exp:control}. Finally, we conduct ablation studies in Section~\ref{exp:abs}. Before delving into the experimental results, we provide an overview of our experimental setup.

\subsection{Experimental Setup}
\paragraph{Environments.} We evaluate the \Model framework in three different environments: 

\vspace{-2mm}
\begin{itemize}

\item \textbf{Webshop} is a well-known environment for online shopping~\citep{yao2023webshopscalablerealworldweb}, where the agent must search for and select products on the website to obtain a final result. Following the setup of AgentBench~\citep{liu2023agentbench} for LLM evaluation, we test the model on the validation split, using the default matching reward as the evaluation metric.
    \item \textbf{ScienceWorld}~\citep{scienceworld2022} is an interactive benchmark designed for embodied science experiments. It places agents in a simulated text-based environment where they must perform elementary science experiments by navigating the environment, manipulating objects, and observing outcomes. The aim is to assess whether AI models can apply scientific knowledge, rather than merely retrieve or assemble information. We evaluate the framework on both seen and unseen splits.
    \item \textbf{Game of 24} is a mathematical game where the agent is given four numbers and must use arithmetic operations (addition, subtraction, multiplication, and division) to make the number 24. For instance, given the input '3, 5, 7, 11,' one possible solution is '$(7 - 3) * (11 - 5) = 24$'. Following~\cite{yao2023treethoughtsdeliberateproblem}, we selected 100 challenging puzzles, specifically those indexed from 901 to 1,000, and the performance metric is the success rate across these puzzles. As shown in Fig.~\ref{fig:train_data_game24} of the Appendix, we use the chain-of-thought prompting technique, prompting the LLM agents to output intermediate steps followed by the final answer. Each step of the solution is considered an action.
\end{itemize}

\paragraph{LLM Setup.}
Our framework requires LLM models to act as agents, generating synthetic task instructions from the environment along with few-shot examples in the prompt context. We also deploy agents to perform these synthetic tasks in the environment, collecting diverse trajectories for further analysis. In this paper, we primarily use the Llama3-70b-instruct model~\citep{dubey2024llama3herdmodels} to synthesize training data for the automatic reward models, as it is open-source, easy to deploy locally, and delivers robust performance. We avoid state-of-the-art commercial models like GPT-4 or Gemini due to their high costs and the complexity of reproducing results caused by frequent model updates, making them less suitable for our research objectives.

To evaluate the performance of various LLM agents, we serve a representative set of LLM APIs locally, balancing model diversity with affordable serving costs. We identify the LLMs by their model family and size. Specifically, these are Llama70B, Llama8B, Mistral7B, and Phi3.8B. We note that these open-source model families are frequently updated, and we provide the current model links in the Appendix~\ref{sec:llmapi}. All models can be easily set up using the vLLM library~\citep{kwon2023efficient} and a single H100 GPU.

\paragraph{Baselines.} 
We implement our \Model framework using different planning algorithms, including Reflexion, Best-of-N, and MCTS, which we denote as \textbf{\Model-R}, \textbf{\Model-B}, and \textbf{\Model-M}, respectively. We limit the maximum number of trajectories our \Model can explore to 10 in the ScienceWorld and Webshop environments to systematically evaluate the pipeline's effectiveness across different LLM agent backbones. We also compare the model with two baselines that do not use reward model guidance: \textbf{Sampling} and \textbf{Greedy}. For the {Game of 24} environment, we follow the setup of a previous study~\citep{yao2023treethoughtsdeliberateproblem} and set the maximum number of explored trajectories to 100. For \textbf{Sampling}, we set the model temperature to 1 and sample action trajectories using chain-of-thought prompting~\citep{wei2023chainofthoughtpromptingelicitsreasoning}. For \textbf{Greedy}, we set the temperature to 0, generating the action sequence with the highest probability. Further implementation details are provided in the Appendix. We will release all the code, model, and data for easy reproduction upon acceptance.

\subsection{Effectiveness for Reward Planning.}
\label{exp:effect}
In this section, we investigate the effectiveness of the framework across different language models~\citep{dubey2024llama3herdmodels,jiang2023mistral7b,abdin2024phi3technicalreporthighly} and various planning algorithms. The results are shown in Table~\ref{tab:comparison}. Based on the table, we have the following observations. First, our proposed pipeline is effective, as it consistently outperforms the \textbf{Sampling} and \textbf{Greedy} baselines across different planning algorithms. Additionally, we observe that the average improvement is more significant on weaker models, such as Phi~\citep{abdin2024phi3technicalreporthighly} and Mistral-7B~\citep{jiang2023mistral7b}, compared to stronger models like Llama3-1-70B~\citep{dubey2024llama3herdmodels}. We believe this is because weaker models explore more low-reward trajectories, providing greater opportunities for the reward model to improve performance.

Among the three planning algorithms, MCTS performs the best on average, likely due to its superior mechanisms for identifying higher-reward trajectories and searching less-explored trajectories. We also notice that Reflexion performs the worst on weaker models like Mistral7B and Phi3.8B. We suspect this is because Reflexion was designed for ChatGPT-family-based agents and requires the LLM agent to possess strong capabilities for learning from trial and error.
Finally, we present qualitative results of different methods in Fig.~\ref{fig:vis_webshop}, where it is clear that our \Model generates better trajectories than the baselines, aided by the guidance of automatic reward models.
In Appendix~\ref{sec:failure}, 
we analyze several failure cases, offer more detailed insights into the limitations of the current approach, and suggest potential improvements in reward modeling.
\input{tables/compare}

\begin{figure}[t]  
   \centering
   \includegraphics[width=1\textwidth]{figures/visualization.pdf}  
   \caption{Two qualitative results of the Webshop task. The figure shows two examples utilizing the advantages of our \Model framework and we are able to correct errors made by existing methods. In the top example, when the search results do not meet the requirements, our \Model method leverages the advantage of the tree structure to backtrack and search again, thereby retrieving the appropriate target item. In contrast, existing methods fail to backtrack when the target item is not found. In the bottom example, by using the \Model to evaluate different states in the environment, our method is able to select the color that offers a higher reward and better meets the requirements when choosing between size and color, rather than mistakenly selecting the wrong size. These two examples sufficiently demonstrate the advantages of our method compared to traditional approaches.}
   \label{fig:vis_webshop}  
\end{figure}

\subsection{Controllable Generation.}
\label{exp:control}
Another benefit of our \Model pipeline is that we can customize our reward targets during inference, allowing us to generate more controllable action sequences, rather than solely maximizing the predicted rewards. Agent fine-tuning methods~\citep{li2023camel,zeng2023agenttuning} find it challenging to achieve this goal since agent behaviors are typically fixed during inference. 
\input{tables/control}
We conducted experiments in the Webshop environment to evaluate the impact of customizable reward targets. In addition to the original objective of maximizing the predicted reward $\mathcal{R}(x,h)$, we defined two additional optimization targets. First, we aimed to minimize the number of actions in the trajectory history, defining the reward target as $\mathcal{R}(x,h) - \text{NumberOfAction}(h)$. Second, we sought to minimize the price of the target product, with a customized target of $\mathcal{R}(x,h) - \text{PriceOfProduct}(h)$. 
Table~\ref{tab:control} presents the results. By applying a length penalty on the reward target for \Model-M, we reduced the average action length from 4.5 to 4 and the average product price from 97.9 to 69.0, while maintaining comparable performance on the default matching reward. Similar performance was observed for \Model-B. Additionally, we provide a qualitative example in Fig.~\ref{fig:control}. From this example, we can see that our customized reward target successfully guided the LLM agent to purchase products with fewer action steps while still finding the target product.

\begin{figure}[t]  
   \centering
   \includegraphics[width=1\textwidth]{figures/control.pdf}  
   \caption{A typical example of customized reward target for shorter trajectory generation. On the left, we show the default greedy decoding generates a long trajectory without finding the target product. In the middle, we show our default reward can guide the LLM agent to generate a correct but long trajectory. On the right, we show our framework with a customized reward target for shorter trajectories, which finds a correct and short trajectory for the target product.}  
   \label{fig:control}  
\end{figure}

\input{tables/ablation}
\subsection{Ablation studies.}
\label{exp:abs}
We conduct ablation studies to investigate the effectiveness of the framework. Specifically, we aim to answer the following questions: 
\textbf{Q1.} Can we train a policy model with fully supervised learning to handle multi-step tasks from the synthesized trajectory data? 
\textbf{Q2.} Can a large, general language model be used as the reward model to perform guidance without automatic reward learning?

We conducted experiments using the ScienceWorld benchmark, and the results are shown in Table~\ref{tab:ablation}. When comparing our pipeline to the SFT model trained using our reward backbone VILA3B, we observed that although the policy model trained through fully supervised learning performed reasonably well (18.6), it still lagged behind the performance of our planning framework (28.3). This suggests that learning a policy model is more challenging than learning a reward model, highlighting the effectiveness of our proposed \Model pipeline (answering \textbf{Q1}).

Next, we replaced our smaller 3B reward model with a much larger language model, Llama3-1-70B, and used few-shot prompting to predict the reward of the extracted trajectories. We found that this larger model also improved performance compared to the default greedy model, demonstrating the effectiveness of our planning framework. However, it still performed worse than our pipeline using automatic reward learning, despite the Llama3-1-70B being about 20 times larger, further showcasing the efficiency and effectiveness of our approach (answering \textbf{Q2}).



We provide additional ablation experiments in the Appendix~\ref{sec:expabl}, including the data quality from various LLMs, reward modeling target and computational efficiency.

==> ICLR_2025_Template/sections/5_conclusion.tex <==
\section{Conclusion}
We propose a framework, \Model, for large language model (LLM) agents to manage tasks that require multi-step decision-making and environmental feedback, such as online shopping or scientific reasoning. This framework allows LLM-based agents to enhance task planning by autonomously learning a reward model from the environment, without the need for human labeling. The method utilizes pre-trained LLM agents to generate diverse action trajectories within an environment, which are then evaluated by a separate LLM based on the task's intent. These evaluations help train a reward model that strengthens the agents' decision-making capabilities. The framework enhances the performance of LLM agents in addressing complex tasks and mitigates issues related to data scarcity and API limitations. Its effectiveness is demonstrated across various benchmarks, representing a significant advancement in the development of AI agents for real-world, multi-step problem-solving.

==> ICLR_2025_Template/tables/ComputationalEfficiency.tex <==
\begin{table*}[!h]
    \centering
    \begin{tabular}{cccccc}
    \toprule
    Backbone  & VILA-3B & VILA-13B & LLaVA-13B &1/5 Data   &1/25 Data \\
    %\midrule
    %GPT-4 & - & 64.8    &  64.4   &   -  &    7.0 & - \\
    \midrule
LLaMA-70B &57.3	&61.2	&44.3	&52.1	&50.6  \\
    LLaMA-8B  &35.7	&34.3	&26.0	&31.4	&29.3   \\
    Mistral-7B &24.5	&26.0	&19.5	&22.6	&21.7    \\
    Phi-3.8B& 20.0	&19.5	&16.7	&17.9	&13.9   \\
    \bottomrule
    \end{tabular}
    \caption{Comparison of reward model selection and data demands on ScienceWorld seen set. 
    }
    \label{tab:Efficiency1}
% \vskip -0.1in
\end{table*}

\begin{table*}[!h]
    \centering
    \begin{tabular}{cccccc}
    \toprule
    Backbone  & VILA-3B & VILA-13B & LLaVA-13B &1/5 Data   &1/25 Data \\
    %\midrule
    %GPT-4 & - & 64.8    &  64.4   &   -  &    7.0 & - \\
    \midrule
    LLaMA-70B &57.0	&60.7	&48.2	&50.0	&47.7  \\
    LLaMA-8B  &28.1	&27.5	&22.2	&26.8	&24.2   \\
    Mistral-7B &21.1	&22.9	&19.2	&21.6	&19.7   \\
    Phi-3.8B& 17.0	&15.3	&13.7	&14.2	&11.7  \\
    \bottomrule
    \end{tabular}
    \caption{Comparison of reward model selection and data demands on ScienceWorld unseen set.} 
    \label{tab:Efficiency2}
% \vskip -0.1in
\end{table*}


==> ICLR_2025_Template/tables/LLMquality.tex <==
\begin{table*}[!h]
    \centering
    \begin{tabular}{lcccc}
    \toprule
    Models    & SciWorld-seen & SciWorld-unseen \\
    \midrule
    Greedy  & 29.9      & 23.8 &  \\
    Llama70B  & 35.7      & 28.1 &  \\
    Llama8B & 32.2 & 24.7  \\
    Mistral7B & 33.7 &  26.5 \\
    Phi3.8B &34.7	&26.9 \\
    \bottomrule
    \end{tabular}
    \caption{Experiments of training data generated from various LLMs.}
    \label{tab:dataquality}
% \vskip -0.1in
\end{table*}


==> ICLR_2025_Template/tables/ablation.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{lcccc}
    \toprule
    Models    & Model Base & ScienceWorld~( seen ) \\
    \midrule
    Greedy  & Phi3.8B      & 9.6 &  \\
    SFT-Policy  & VILA3B      & 18.6 &  \\
    \midrule
    \Model-B w/o R &      \multirow{2}{*}{Llama70B and Phi3.8B} & 16.0  \\
    \Model-M w/o R &  &  26.5 \\
    \midrule
    \Model-B  &  \multirow{2}{*}{VILA3B and Phi3.8B} & 20.0 \\
    \Model-M  & & 28.3 \\
    \bottomrule
    \end{tabular}
    \caption{Ablation study of the proposed framework. Our \Model framework is more effective than directly finding a policy model and using the general LLM for reward generation.}
    \label{tab:ablation}
% \vskip -0.1in
\end{table*}

==> ICLR_2025_Template/tables/alfworld.tex <==
\begin{table*}[!h]
    \centering
    \begin{tabular}{lcccc}
    \toprule
    Models    & ALFWorld-std & ALFWorld-dev \\
    \midrule
    Sampling  & 0.13      & 0.14 &  \\
    Greedy  & 0.18      & 0.30 &  \\
    ARMAP-R & 0.22 & 0.35  \\
    ARMAP-B & 0.30 &  0.45 \\
    \bottomrule
    \end{tabular}
    \caption{Experimental Results on ALFWorld.}
    \label{tab:alfworld}
% \vskip -0.1in
\end{table*}

==> ICLR_2025_Template/tables/api_model.tex <==
\begin{table*}[!h]
    \centering
    \begin{tabular}{lcccc}
    \toprule
    GPT-4o    & Std & Dev \\
    \midrule
    Sampling  & 0.74      & 0.88 &  \\
    Greedy  & 0.82      & 0.90 &  \\
    ARMAP-B & 0.84 & 0.95  \\
    \bottomrule
    \end{tabular}
    \caption{Experiments of using the proprietary model on ALFWorld}
    \label{tab:api_model}
\end{table*}


==> ICLR_2025_Template/tables/clinicalagent.tex <==
\begin{table*}[!h]
    \centering
    \begin{tabular}{lccc}
    \toprule
    Models    & AgentClinic-MedQA  \\
    \midrule
    Sampling  & 11.89  \\
    Greedy  & 14.02 \\
    ARMAP-B & 44.33 \\
    \bottomrule
    \end{tabular}
    \caption{Experiments Results on AgentClinic.}
    \label{tab:clinic}
% \vskip -0.1in
\end{table*}

==> ICLR_2025_Template/tables/compare.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{llccccc}
    \toprule
    \multirow{2}{*}{Backbone}    & \multirow{2}{*}{Algorithms} &  \multirow{2}{*}{Webshop} & \multicolumn{2}{c}{ScienceWorld}   &  \multirow{2}{*}{Game24} &  \multirow{2}{*}{Average}  \\
      & & & seen & unseen \\
    \midrule
    \multirow{5}{*}{Llama70B} 
      & Sampling & 52.0 &53.9 & 50.6 &  9.6 & 38.0 \\
      & Greedy   & 50.4 &57.2 & 55.1 &  6.0 & 37.5\\
      & \Model-R & 56.5 &\textbf{59.0} & 56.7 & 16.0 & 43.5 \\
      & \Model-B & 62.0 &57.3 & \textbf{57.0} &  19.0 & 46.1 \\
      & \Model-M & \textbf{66.8} &58.2 & 55.9 &  \textbf{24.0} & \textbf{49.3} \\
    \midrule
    \multirow{5}{*}{Llama8B} 
      & Sampling   & 56.4 &24.5 & 20.6 &  2.0 & 27.0\\
      & Greedy    & 57.7 &29.9 & 23.8 &  2.0 & 28.9 \\
      & \Model-R &  58.3 & 31.2 & 28.0 & 6.0  & 31.3 \\
      & \Model-B  & 59.3 &\textbf{35.7} & \textbf{28.1} &  \textbf{11.0} & \textbf{34.1} \\
      & \Model-M & \textbf{60.2} &32.5 & 24.9  &  9.0 & 32.6\\
    \midrule
    \multirow{5}{*}{Mistral7B}  
      & Sampling & 17.7 &18.4 & 17.1 &  1.0 & 12.2 \\
      & Greedy &37.2  & 21.1 & 19.6 &  1.0 & 19.5 \\
      & \Model-R & 54.1 & 21.7 & 19.7  & 2.0  & 25.6\\
      & \Model-B & 54.4 &24.5 & 21.2 &  2.0 & 26.4 \\
      & \Model-M & \textbf{58.2} &\textbf{30.0} & \textbf{23.4} &  \textbf{4.0} & \textbf{29.6} \\
    \midrule
    \multirow{5}{*}{Phi3.8B} 
      & Sampling & 34.7 & 10.0 & 7.6 & 2.0 & 15.2 \\
      & Greedy & 42.4 & 9.5 & 6.5 &  2.1 & 17.5 \\
      & \Model-R & 53.3 & 9.6 & 7.2 &  4.0 & 21.9\\
      & \Model-B & 52.1 &20.0 & 17.0 &  9.0 & 26.5 \\
      & \Model-M & \textbf{53.7}  &\textbf{28.3} & \textbf{24.3} &  \textbf{10.0} & \textbf{30.0} \\
    \bottomrule
    \end{tabular}
    \caption{Effectiveness of the proposed method on different benchmarks. Our \Model framework consistently outperforms the baselines across different language models. 
    }
    \label{tab:comparison}
\end{table*}


==> ICLR_2025_Template/tables/control.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{llcccc}
    \toprule
    Algorithms & Action$\downarrow$ & Price $\downarrow$  &  Reward $\uparrow$ \\
    \midrule
      Greedy                  &  4.6   &  102.4   & 50.4 \\
      \Model-B                &  4.7   &  102.2   & 62.0 \\
      \Model-M                &  4.5   &  97.9    & 66.8 \\
      \midrule
      \Model-B+Length-Penalty &   3.9 &  98.8 & 60.3 \\
      \Model-M+Length-penalty &       4.0  & 102.1  & 65.5   \\
      \midrule
      \Model-B+Price-penalty & 5.0 & 65.5 & 57.5 \\
      \Model-M+Price-penalty & 4.3  &  69.0  & 62.4 \\
    \bottomrule
    \end{tabular}
    \caption{Controllable Trajectory Generation. We show that we can generate controllable trajectories like shorter action lengths and lower prices by customizing reward targets. We use Llama70B as the default API for action prediction.}
    \vspace{-2em}
    \label{tab:control}
\end{table}

==> ICLR_2025_Template/tables/generalization.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{lccc}
    \toprule
    Backbone    & Models & Room2Room & ScienceWorld \\
    \midrule
    \multirow{4}{*}{Mistral 7B}  & -      & \\
      & Sampling & \\
      & Reflexion & \\
      & MCTS \\
    \midrule
    \multirow{4}{*}{Llama38B}   & -      & \\
       & Sampling & \\
      & Reflexion & \\
      & MCTS \\
    \midrule
    \multirow{4}{*}{Llama370B}   & -      & \\
       & Sampling & \\
      & Reflexion & \\
      & MCTS \\
    \midrule
    \multirow{4}{*}{Gemini}   & -      & \\
       & Sampling & \\
      & Reflexion & \\
      & MCTS \\
    \midrule
    \multirow{4}{*}{GPT4-V}   & -      & \\
       & Sampling & \\
      & Reflexion & \\
      & MCTS \\
    \midrule
    \end{tabular}
    \caption{Generalization of the proposed method on benchmarks.}
    \label{tab:dataset_comparison}
% \vskip -0.1in
\end{table*}

==> ICLR_2025_Template/tables/overhead.tex <==
\begin{table*}[!h]
    \centering
    \begin{tabular}{cccc}
    \toprule
    Tasks	&Samples	&Tokens	&Tokens per Sample  \\
    %\midrule
    %GPT-4 & - & 64.8    &  64.4   &   -  &    7.0 & - \\
    \midrule
    ScienceWorld	&4064	&2541255	&625\\
    Webshop	&2436	&6645746	&2728 \\
    Game of 24	&37885	&12846182	&339 \\
    \bottomrule
    \end{tabular}
    \caption{Tokens of data generation in three different tasks. 
    }
    \label{tab:overhead}
% \vskip -0.1in
\end{table*}



==> ICLR_2025_Template/tables/rewardtarget.tex <==
\begin{table*}[!h]
    \centering
    \begin{tabular}{llcccc}
    \toprule
    \multirow{2}{*}{Backbone}    & \multirow{2}{*}{Algorithms} &  \multicolumn{2}{c}{Classification} & \multicolumn{2}{c}{Comparative}    \\
       && Seen & Unseen & Seen & Unseen \\
    \midrule
    \multirow{2}{*}{LLaMA-70B} 
      & \Model-R &57.0&55.4&59.0&56.7  \\
      & \Model-B &47.2&43.3&57.3&57.0  \\
    \midrule
    \multirow{2}{*}{LLaMA-8B} 
      & \Model-R &29.0&24.2&31.2&28.0   \\
      & \Model-B  &27.5&22.2&35.7&28.1 \\
    \midrule
    \multirow{2}{*}{Mistral-7B}  
      & \Model-R & 17.8 &18.2  &21.7   &19.7   \\
      & \Model-B & 19.1  &17.3  &24.5  &21.1    \\
    \midrule
    \multirow{2}{*}{Phi-3.8B} 
      & \Model-R &8.6   &4.8  &9.6  & 7.2  \\
      & \Model-B &17.7  &13.7  &20.0   &17.0   \\
    \bottomrule
    \end{tabular}
    \caption{Comparison of the Classification target and Comparison target on ScienceWorld. 
    }
    \label{tab:rewardtarget}
% \vskip -0.1in
\end{table*}


==> ICLR_2025_Template/tables/visualinfo.tex <==
\begin{table*}[!h]
    \centering
    \begin{tabular}{cccc}
    \toprule
    Backbone    & Algorithms & w/o visual	&w/ visual   \\
    \midrule
    \multirow{2}{*}{LLaMA-70B} 
      & \Model-R &56.1	&56.5 \\
      & \Model-B &61.6	&62.0\\
    \midrule
    \multirow{2}{*}{Mistral-7B}  
      & \Model-R & 53.6	&54.1  \\
      & \Model-B & 51.3	&54.4  \\
    \bottomrule
    \end{tabular}
    \caption{Ablation of the visual input. 
    }
    \label{tab:visualinfo}
% \vskip -0.1in
\end{table*}

==> tables/generalization.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{lccc}
    \toprule
    Backbone    & Models & Room2Room & ScienceWorld \\
    \midrule
    \multirow{4}{*}{Mistral 7B}  & -      & \\
      & Sampling & \\
      & Reflexion & \\
      & MCTS \\
    \midrule
    \multirow{4}{*}{Llama38B}   & -      & \\
       & Sampling & \\
      & Reflexion & \\
      & MCTS \\
    \midrule
    \multirow{4}{*}{Llama370B}   & -      & \\
       & Sampling & \\
      & Reflexion & \\
      & MCTS \\
    \midrule
    \multirow{4}{*}{Gemini}   & -      & \\
       & Sampling & \\
      & Reflexion & \\
      & MCTS \\
    \midrule
    \multirow{4}{*}{GPT4-V}   & -      & \\
       & Sampling & \\
      & Reflexion & \\
      & MCTS \\
    \midrule
    \end{tabular}
    \caption{Generalization of the proposed method on benchmarks.}
    \label{tab:dataset_comparison}
% \vskip -0.1in
\end{table*}
